Rainbow Memory: Continual Learning with a Memory of Diverse Samples

Continual learning is a realistic learning scenario for AI models. Prevalent scenario of continual learning, however, assumes disjoint sets of classes as tasks and is less realistic rather artificial. Instead, we focus on 'blurry' task boundary; where tasks shares classes and is more realistic and practical. To address such task, we argue the importance of diversity of samples in an episodic memory. To enhance the sample diversity in the memory, we propose a novel memory management strategy based on per-sample classification uncertainty and data augmentation, named Rainbow Memory (RM). With extensive empirical validations on MNIST, CIFAR10, CIFAR100, and ImageNet datasets, we show that the proposed method significantly improves the accuracy in blurry continual learning setups, outperforming state of the arts by large margins despite its simplicity. Code and data splits will be available in https://github.com/clovaai/rainbow-memory.

==> tables/abl_data_augmentation.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{graphicx}
% \begin{table}[]
% \centering
% \caption{Comparison of last accuracy (A5 ($\uparrow$), \%) over methods with data augmentations in CIFAR10-Blurry10-Online.}
% \label{tab:abl-data-augmentation}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{@{}cccccc@{}}
% \toprule
% Methods & None & CutMix & RandAug & AutoAug & \begin{tabular}[c]{@{}l@{}}CutMix\\ +AutoAug\end{tabular}\\ 
% \midrule
% \multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=200}}\\
% % EWC   & 40.07$\pm$2.14 & 41.92$\pm$1.07 & 44.79$\pm$0.69 & 48.32$\pm$3.51 & 50.39$\pm$1.24\\
% % Rwalk & 38.66$\pm$1.52 & 41.35$\pm$2.25 & 46.57$\pm$2.95 & 48.71$\pm$2.76 & 51.8$\pm$1.64\\
% % iCaRL & 37.43$\pm$1.31 & 37.99$\pm$3.80 & 38.42$\pm$1.48 & 41.83$\pm$2.36 & 43.39$\pm$2.28\\
% % GDumb & 33.35$\pm$2.06 & 35.85$\pm$1.03 & 37.15$\pm$2.04 & 38.46$\pm$1.14 & 41.49$\pm$1.19\\
% % BiC   & 33.29$\pm$0.86 & 33.29$\pm$0.86 & 27.16$\pm$2.71 & 29.79$\pm$3.17 & 31.2$\pm$0.73\\
% % \memname (Ours) & \textbf{44.41$\pm$1.40} & \textbf{45.90$\pm$2.42} & \textbf{49.92$\pm$2.97} & \textbf{55.37$\pm$2.23} & \textbf{54.61$\pm$1.62}\\
% EWC   & 40.0$\pm$2.1 & 41.9$\pm$1.0 & 44.7$\pm$0.6 & 48.3$\pm$3.5 & 50.3$\pm$1.2\\
% Rwalk & 38.6$\pm$1.5 & 41.3$\pm$2.2 & 46.5$\pm$2.9 & 48.7$\pm$2.7 & 51.8$\pm$1.6\\
% iCaRL & 37.4$\pm$1.3 & 37.9$\pm$3.8 & 38.4$\pm$1.4 & 41.8$\pm$2.3 & 43.3$\pm$2.2\\
% GDumb & 33.3$\pm$2.0 & 35.8$\pm$1.0 & 37.1$\pm$2.0 & 38.4$\pm$1.1 & 41.4$\pm$1.1\\
% BiC   & 33.2$\pm$0.8 & 33.2$\pm$0.8 & 27.1$\pm$2.7 & 29.7$\pm$3.1 & 31.2$\pm$0.7\\
% \cmidrule(lr){1-6} 
% \memname (Ours) & \textbf{44.4$\pm$1.4} & \textbf{45.9$\pm$2.4} & \textbf{49.9$\pm$2.9} & \textbf{55.3$\pm$2.2} & \textbf{54.6$\pm$1.6}\\
% \midrule
% \multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=500}}\\
% EWC   & 55.6$\pm$4.6 & 56.2$\pm$0.7 & 60.0$\pm$5.3 & 64.8$\pm$0.6 & 67.5$\pm$0.9\\
% Rwalk & 53.6$\pm$3.1 & 57.5$\pm$1.4 & 62.5$\pm$3.0 & 64.7$\pm$1.0 & 67.2$\pm$1.5\\
% iCaRL & 45.9$\pm$3.0 & 46.9$\pm$1.4 & 51.3$\pm$1.1 & 51.6$\pm$2.8 & 56.6$\pm$1.2\\
% GDumb & 46.7$\pm$1.5 & 49.4$\pm$1.0 & 54.3$\pm$1.4 & 55.9$\pm$1.4 & 58.2$\pm$2.7\\
% BiC   & 42.0$\pm$2.4 & 42.0$\pm$2.4 & 38.6$\pm$2.8 & 38.7$\pm$1.5 & 38.4$\pm$2.5\\
% \cmidrule(lr){1-6} 
% \memname (Ours) & \textbf{60.8$\pm$0.8} & \textbf{62.0$\pm$3.5} & \textbf{68.6$\pm$0.7} & \textbf{69.6$\pm$2.9} & \textbf{71.1$\pm$0.1}\\
% \midrule
% \multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=1,000}}\\
% % EWC   & 68.67$\pm$0.95 & 70.5$\pm$0.68 & 73.02$\pm$0.51 & 75.11$\pm$2.24 & 75.27$\pm$0.08\\
% % Rwalk & 68.20$\pm$1.86 & 69.72$\pm$1.02 & 73.56$\pm$0.13 & 76.09$\pm$4.08 & 76.22$\pm$0.41\\
% % iCaRL & 53.60$\pm$2.82 & 56.11$\pm$2.69 & 57.7$\pm$0.73 & 62.55$\pm$6.19  & 63.88$\pm$1.15\\
% % GDumb & 59.12$\pm$0.39 & 64.26$\pm$1.21 & 67.54$\pm$1.31 & 67.6$\pm$2.28 & 70.39$\pm$0.65\\
% % BiC   & 47.81$\pm$3.04 & 47.81$\pm$3.04 & 45.38$\pm$7.75 & 45.68$\pm$5.87 & 48.59$\pm$5.01\\
% % \memname (Ours) & \textbf{70.93$\pm$1.57} & \textbf{74.76$\pm$0.69} & \textbf{76.4$\pm$0.38} & \textbf{77.55$\pm$0.71} & \textbf{78.04$\pm$0.50}\\ \bottomrule
% EWC   & 68.6$\pm$0.9 & 70.5$\pm$0.6 & 73.0$\pm$0.5 & 75.1$\pm$2.2 & 75.2$\pm$0.0\\
% Rwalk & 68.2$\pm$1.8 & 69.7$\pm$1.0 & 73.5$\pm$0.1 & 76.0$\pm$4.0 & 76.2$\pm$0.4\\
% iCaRL & 53.6$\pm$2.8 & 56.1$\pm$2.6 & 57.7$\pm$0.7 & 62.5$\pm$6.1 & 63.8$\pm$1.1\\
% GDumb & 59.1$\pm$0.3 & 64.2$\pm$1.2 & 67.5$\pm$1.3 & 67.6$\pm$2.2 & 70.3$\pm$0.6\\
% BiC   & 47.8$\pm$3.0 & 47.8$\pm$3.0 & 45.3$\pm$7.7 & 45.6$\pm$5.8 & 48.5$\pm$5.0\\
% \cmidrule(lr){1-6} 
% \memname (Ours) & \textbf{70.9$\pm$1.5} & \textbf{74.7$\pm$0.7} & \textbf{76.4$\pm$0.4} & \textbf{77.5$\pm$0.7} & \textbf{78.0$\pm$0.5}\\ \bottomrule
% % \textbf{\our} & 70.9 $\pm$ 1.6 & 74.8 $\pm$ 0.7 & 77.6 $\pm$ 0.7 & 76.4 $\pm$ 0.4 \\ \bottomrule
% \end{tabular}%
% }
% \vspace{-1.0em}
% \end{table}





\begin{table*}[tp]
\centering
\caption{Comparison of last accuracy (A5 ($\uparrow$), \%) over methods with data augmentations in CIFAR10-Blurry10-Online. The results on $K=1,000$ is reported in the supplementary material. `CM+AA' refers to CutMix+AutoAug.}
%\yj{table font 너무 작은거 같은데 1000은 supple로 빼는게 어떤가요?}}
\label{tab:abl-data-augmentation}
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{@{}crrrrrrrrrr@{}}
\toprule
& \multicolumn{5}{c}{K=200} & \multicolumn{5}{c}{ K=500} \\
% & \multicolumn{5}{c}{\bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=1000}} \\
Methods & None & CutMix & RandAug & AutoAug & \begin{tabular}[c]{@{}l@{}}CM+AA\end{tabular} & None & CutMix & RandAug & AutoAug & \begin{tabular}[c]{@{}l@{}}CM+AA\end{tabular} \\
% & None & CutMix & RandAug & AutoAug & \begin{tabular}[c]{@{}l@{}}CutMix\\ +AutoAug\end{tabular} \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-6} \cmidrule(lr){7-11} 
% EWC   & 40.07$\pm$2.14 & 41.92$\pm$1.07 & 44.79$\pm$0.69 & 48.32$\pm$3.51 & 50.39$\pm$1.24\\
% Rwalk & 38.66$\pm$1.52 & 41.35$\pm$2.25 & 46.57$\pm$2.95 & 48.71$\pm$2.76 & 51.8$\pm$1.64\\
% iCaRL & 37.43$\pm$1.31 & 37.99$\pm$3.80 & 38.42$\pm$1.48 & 41.83$\pm$2.36 & 43.39$\pm$2.28\\
% GDumb & 33.35$\pm$2.06 & 35.85$\pm$1.03 & 37.15$\pm$2.04 & 38.46$\pm$1.14 & 41.49$\pm$1.19\\
% BiC   & 33.29$\pm$0.86 & 33.29$\pm$0.86 & 27.16$\pm$2.71 & 29.79$\pm$3.17 & 31.2$\pm$0.73\\
% \memname (Ours) & \textbf{44.41$\pm$1.40} & \textbf{45.90$\pm$2.42} & \textbf{49.92$\pm$2.97} & \textbf{55.37$\pm$2.23} & \textbf{54.61$\pm$1.62}\\
EWC   & 40.0$\pm$2.1 & 41.9$\pm$1.0 & 44.7$\pm$0.6 & 48.3$\pm$3.5 & 50.3$\pm$1.2 
& 55.6$\pm$4.6 & 56.2$\pm$0.7 & 60.0$\pm$5.3 & 64.8$\pm$0.6 & 67.5$\pm$0.9 \\
% & 68.6$\pm$0.9 & 70.5$\pm$0.6 & 73.0$\pm$0.5 & 75.1$\pm$2.2 & 75.2$\pm$0.0 \\
Rwalk & 38.6$\pm$1.5 & 41.3$\pm$2.2 & 46.5$\pm$2.9 & 48.7$\pm$2.7 & 51.8$\pm$1.6
& 53.6$\pm$3.1 & 57.5$\pm$1.4 & 62.5$\pm$3.0 & 64.7$\pm$1.0 & 67.2$\pm$1.5 \\
% & 68.2$\pm$1.8 & 69.7$\pm$1.0 & 73.5$\pm$0.1 & 76.0$\pm$4.0 & 76.2$\pm$0.4 \\
iCaRL & 37.4$\pm$1.3 & 37.9$\pm$3.8 & 38.4$\pm$1.4 & 41.8$\pm$2.3 & 43.3$\pm$2.2
& 45.9$\pm$3.0 & 46.9$\pm$1.4 & 51.3$\pm$1.1 & 51.6$\pm$2.8 & 56.6$\pm$1.2 \\
% & 53.6$\pm$2.8 & 56.1$\pm$2.6 & 57.7$\pm$0.7 & 62.5$\pm$6.1 & 63.8$\pm$1.1 \\
GDumb & 33.3$\pm$2.0 & 35.8$\pm$1.0 & 37.1$\pm$2.0 & 38.4$\pm$1.1 & 41.4$\pm$1.1
& 46.7$\pm$1.5 & 49.4$\pm$1.0 & 54.3$\pm$1.4 & 55.9$\pm$1.4 & 58.2$\pm$2.7 \\
% & 59.1$\pm$0.3 & 64.2$\pm$1.2 & 67.5$\pm$1.3 & 67.6$\pm$2.2 & 70.3$\pm$0.6 \\
BiC   & 33.2$\pm$0.8 & 33.2$\pm$0.8 & 27.1$\pm$2.7 & 29.7$\pm$3.1 & 31.2$\pm$0.7
& 42.0$\pm$2.4 & 42.0$\pm$2.4 & 38.6$\pm$2.8 & 38.7$\pm$1.5 & 38.4$\pm$2.5 \\
% & 47.8$\pm$3.0 & 47.8$\pm$3.0 & 45.3$\pm$7.7 & 45.6$\pm$5.8 & 48.5$\pm$5.0 \\
\cmidrule(lr){1-11} 
\textbf{\our} & \textbf{44.4$\pm$1.4} & \textbf{45.9$\pm$2.4} & \textbf{49.9$\pm$2.9} & \textbf{55.3$\pm$2.2} & \textbf{54.6$\pm$1.6}
& \textbf{60.8$\pm$0.8} & \textbf{62.0$\pm$3.5} & \textbf{68.6$\pm$0.7} & \textbf{69.6$\pm$2.9} & \textbf{71.1$\pm$0.1} \\ \bottomrule
% &  \textbf{70.9$\pm$1.5} & \textbf{74.7$\pm$0.7} & \textbf{76.4$\pm$0.4} & \textbf{77.5$\pm$0.7} & \textbf{78.0$\pm$0.5} \\ \bottomrule
% \textbf{\our} & 70.9 $\pm$ 1.6 & 74.8 $\pm$ 0.7 & 77.6 $\pm$ 0.7 & 76.4 $\pm$ 0.4 \\ \bottomrule
\end{tabular}%
}
\vspace{-1.0em}
\end{table*}

==> tables/abl_memory_update_rule.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{graphicx}
% \begin{table}[]
% \centering
% \caption{Comparison over Memory Update Rules in CIFAR10-Blurry10-Online.}
% \label{tab:memory_update_rule}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{@{}ccccccccc@{}}
% \toprule
%  & \multicolumn{4}{c}{K=200} & \multicolumn{4}{c}{K=1000} \\
% Mem-Udt. & None & CutMix & RandAug & \begin{tabular}[c]{@{}l@{}}CutMix+\\ RandAug\end{tabular} & None & CutMix & RandAug & \begin{tabular}[c]{@{}l@{}}CutMix+\\ RandAug\end{tabular} \\ 
% \cmidrule(lr){1-1} \cmidrule(lr){2-5} \cmidrule(lr){6-9} 
% Random & 24.08 & 23.7 & 23.74 & 23.96 & 49.22 & 55.30 & 61.50 & 61.29\\
% Reservoir & 35.64 & 38.26 & 37.27 & 44.09 & 62.42 & 63.15 & 73.72 & 74.83 \\
% Balanced & 44.35 & 40.29 & 51.05 & 50.74 & 67.84 & 70.71 & 76.02 & 78.07 \\
% Prototype & 34.57 & 35.05 & 29.33 & 28.23 & 51.43 & 44.40 & 45.1 & 32.78  \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-5} \cmidrule(lr){6-9} 
% \textbf{\memname} & 41.65 & 40.41 & 48.69 & 50.72 & 67.71 & 70.18 & 77.36 & 78.27 \\ \bottomrule
% \end{tabular}%
% }
% \end{table}


% backup including randaug+cutmix
% \begin{tabular}{@{}crrrr@{}}
% \toprule
% %  & \multicolumn{4}{c}{K=200} \\ 
% Methods & None & CutMix & RandAug & \begin{tabular}[c]{@{}l@{}}CutMix\\ +RandAug\end{tabular} \\ \midrule
% \multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=200}}\\
% Random    & 24.1 $\pm$ 1.4 & 24.0 $\pm$ 1.0 & 25.6 $\pm$ 1.6 & 24.8 $\pm$ 1.2 \\
% Reservoir & 38.0 $\pm$ 2.2 & 39.1 $\pm$ 0.8 & 39.7 $\pm$ 2.9 & 46.6 $\pm$ 2.6 \\
% %Balanced  & 44.3 $\pm$ 0.2 & 43.0 $\pm$ 2.5 & 48.2 $\pm$ 2.6 & 49.1 $\pm$ 3.4 \\
% Prototype & 34.6 $\pm$ 0.5 & 33.8 $\pm$ 1.9 & 30.1 $\pm$ 0.7 & 28.2 $\pm$ 4.0 \\
% % \textbf{\memname (Ours)}& 43.0 $\pm$ 1.9 & 42.4 $\pm$ 1.8 & 47.9 $\pm$ 0.7 & 48.4 $\pm$ 3.4 \\ 
% \memname (Ours) & \textbf{43.8 $\pm$ 1.2} & \textbf{42.4 $\pm$ 1.8} & \textbf{47.9 $\pm$ 0.7} & \textbf{48.4 $\pm$ 3.4} \\ 

% \midrule
% %  & \multicolumn{4}{c}{K=1000} \\
% Methods. & None & CutMix & RandAug & \begin{tabular}[c]{@{}l@{}}CutMix\\ +RandAug\end{tabular} \\ \midrule
% \multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=1000}}\\
% Random            & 46.7 $\pm$ 2.5 & 52.5 $\pm$ 4.2 & 57.2 $\pm$ 3.8 & 57.0 $\pm$ 4.1 \\
% Reservoir         & 64.6 $\pm$ 4.2 & 67.2 $\pm$ 5.3 & 73.9 $\pm$ 0.8 & 74.9 $\pm$ 0.3 \\
% %Balanced          & 65.0 $\pm$ 4.6 & 71.9 $\pm$ 4.3 & 75.1 $\pm$ 2.2 & 77.0 $\pm$ 1.3 \\
% Prototype         & 48.1 $\pm$ 5.7 & 41.1 $\pm$ 4.1 & 40.0 $\pm$ 4.5 & 32.3 $\pm$ 2.6 \\
% \memname (Ours) &\textbf{ 64.7 $\pm$ 4.1} & \textbf{71.8 $\pm$ 4.3} & \textbf{75.8 $\pm$ 2.3} & \textbf{76.8 $\pm$ 0.7} \\
% % \textbf{\memname (Ours)} & 65.4$\pm$4.6 & 71.5$\pm$4.0 & 75.7$\pm$1.9 & 77.2$\pm$1.0 \\
% \bottomrule
% \end{tabular}%

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}





\begin{table}[h]
\centering
\caption{Comparison of last accuracy (A5 ($\uparrow$), \%) over memory update methods without data augmentations in CIFAR10-Blurry10-Online. `CM+AA' refers to CutMix+AutoAug.}
\label{tab:memory_update_rule}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}crrrrrr@{}}
\toprule
& \multicolumn{3}{c}{K=200} 
& \multicolumn{3}{c}{K=1,000} \\ 
Methods & None & CutMix & CM+AA
& None & CutMix & CM+AA \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7}
Random & 24.1 $\pm$ 1.4 & 24.0 $\pm$ 1.0 & 22.4 $\pm$ 0.8  
& 46.7 $\pm$ 2.5 & 52.5 $\pm$ 4.2 & 52.7 $\pm$ 2.8\\
Reservoir & 38.0 $\pm$ 2.2 & 39.1 $\pm$ 0.8 & 49.4 $\pm$ 1.8 
& 64.6 $\pm$ 4.2 & 67.2 $\pm$ 5.3 & 75.5 $\pm$ 0.0\\
Prototype & 34.6 $\pm$ 0.5 & 33.8 $\pm$ 1.9 & 26.5 $\pm$ 3.9
& 48.1 $\pm$ 5.7 & 41.1 $\pm$ 4.1 & 29.3 $\pm$ 1.5 \\
\cmidrule(lr){1-7} 
\textbf{Uncertainty} (\memname) & \textbf{43.8 $\pm$ 1.2}
& \textbf{42.4 $\pm$ 1.8} 
& \textbf{52.2 $\pm$ 1.3} 
& \textbf{64.7 $\pm$ 4.1} & \textbf{71.8 $\pm$ 4.3} & \textbf{76.1 $\pm$ 1.1}\\ \bottomrule

% \midrule
% %  & \multicolumn{4}{c}{K=1000} \\
% % Methods. & None & CutMix & RandAug \\ \midrule
% \multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=1000}}\\
% Random & 46.7 $\pm$ 2.5 & 52.5 $\pm$ 4.2 & 52.7 $\pm$ 2.8  \\
% Reservoir         & 64.6 $\pm$ 4.2 & 67.2 $\pm$ 5.3 & 75.5 $\pm$ 0.0  \\
% Prototype         & 48.1 $\pm$ 5.7 & 41.1 $\pm$ 4.1 & 29.3 $\pm$ 1.5  \\

% \cmidrule(lr){1-4} 
% \textbf{\memname} & \textbf{64.7 $\pm$ 4.1} & \textbf{71.8 $\pm$ 4.3} & \textbf{76.1 $\pm$ 1.1} \\
% \bottomrule
\end{tabular}%
}
\vspace{-1.0em}
\end{table}


% \begin{table}[t]
% \centering
% \caption{Comparison of last accuracy (A5 ($\uparrow$), \%) over memory update methods in CIFAR10-Blurry10-Online.}
% \label{tab:memory_update_rule}
% \resizebox{0.72\linewidth}{!}{%
% \begin{tabular}{@{}crr@{}}
% \toprule
% Methods & \multicolumn{1}{c}{\bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=200}} & \multicolumn{1}{c}{\bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=1,000}}\\ \midrule
% % Unbalanced Random & 24.1 $\pm$ 1.4 & 46.7 $\pm$ 2.5 \\
% Random & 24.1 $\pm$ 1.4 & 46.7 $\pm$ 2.5 \\
% Reservoir         & 38.0 $\pm$ 2.2 & 64.6 $\pm$ 4.2 \\
% Prototype~\cite{icarl}         & 34.6 $\pm$ 0.5 & 48.1 $\pm$ 5.7 \\
% % Balanced Random   & 44.3 $\pm$ 0.2 & 65.0 $\pm$ 4.6 \\
% \cmidrule(lr){1-3}
% \textbf{\memname w/o DA}          & 43.8 $\pm$ 1.2 & 64.7 $\pm$ 4.1 \\
% \textbf{\our}       & \bf{52.2 $\pm$ 1.3} & \bf{76.1 $\pm$ 1.1} \\ \bottomrule
% \end{tabular}
% }
% \end{table}

==> tables/aug_combs.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table}[]
% \centering
% \caption{Comparison of Augmentation Combinations.}
% \label{tab:aug_combs}
% \resizebox{.5\textwidth}{!}{
% \begin{tabular}{lllll}
% \hline
% Methods & \begin{tabular}[c]{@{}l@{}}CutMix+\\ RandAug\end{tabular} & \begin{tabular}[c]{@{}l@{}}CutMix+\\ AutoAug\end{tabular} & Comb3 & Comb4 \\ \hline
% EWC &  00.00 & 00.00 74.97 & 75.36 &\\
% Rwalk &  00.00 & 00.00 75.14 & 76.39 &\\
% iCaRL & 00.00 & 00.00  58.73 & 64.55 &\\
% % ER-FAIR & 00.00 & 00.00 & 00.00 & 00.00 \\
% GDumb &  00.00 & 00.00 71.28 & 71.14 &\\
% BiC &  00.00 & 00.00 52.65 & 52.42 &\\
% \textbf{\memname} (Ours) & 00.00 & 78.56 & 00.00 & 00.00 \\
% \textbf{\memname} (RandAug) & 00.00 & 00.00 & 00.00 & 00.00 \\
% \hline
% \end{tabular}
% }
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Comparison of Augmentation Combinations.}
\label{tab:aug_combs}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}llll@{}}
\toprule
Methods & \begin{tabular}[c]{@{}l@{}}CutMix\\ +AutoAug\end{tabular} & \begin{tabular}[c]{@{}l@{}}CutMix\\ +RandAug\end{tabular} & \begin{tabular}[c]{@{}l@{}}CutMix\\ +RandAug\_Hard\end{tabular} \\ \midrule
EWC          & 75.36 & 74.97 & 00.00 \\
Rwalk        & 76.39 & 75.14 & 00.00 \\
iCaRL        & 64.55 & 58.73 & 00.00 \\
GDumb        & 71.14 & 71.28 & 00.00 \\
BiC          & 52.42 & 52.65 & 00.00 \\
DAS-DA       & 00.00 & 00.00 & 00.00 \\ \bottomrule
\end{tabular}%
% }
\end{table}

==> tables/cifar10-blurry-disjoint.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{Comparison of last accuracy (A5 ($\uparrow$), \%) over benchmarks \{Disjoint (0\%), Blurry (10\%), and Blurry (30\%)\} and training setups \{Online and Offline\} on CIFAR10 (K=500).}
\label{tab:cifar10-blurry-disjoint}
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{@{}crrrrrr@{}}
\toprule
 & \multicolumn{2}{c}{Blurry0 (=Disjoint)} & \multicolumn{2}{c}{Blurry10} &  \multicolumn{2}{c}{Blurry30} \\
Methods & \multicolumn{1}{c}{Online} & \multicolumn{1}{c}{Offline} & \multicolumn{1}{c}{Online} & \multicolumn{1}{c}{Offline}  & \multicolumn{1}{c}{Online} & \multicolumn{1}{c}{Offline} \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
% \multicolumn{6}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=500}}\\
EWC               & 55.66 $\pm$ 1.18 & 64.00 $\pm$ 1.34 & 55.65 $\pm$ 4.60 & \textbf{78.67 $\pm$ 1.06} & 60.57 $\pm$ 1.15 & 85.00 $\pm$0.42 \\
Rwalk             & 55.91 $\pm$ 1.85 & 65.04 $\pm$ 0.11 & 53.66 $\pm$ 3.18 & 78.59 $\pm$ 1.37 & 59.03 $\pm$ 0.05 & \textbf{85.18 $\pm$ 0.57} \\
iCaRL             & 40.70 $\pm$ 5.13 & \textbf{65.61 $\pm$ 2.57} & 45.98 $\pm$ 3.04 & 57.07 $\pm$ 2.74 & 48.11 $\pm$ 4.63 & 64.90 $\pm$ 7.95 \\
GDumb             & 50.37 $\pm$ 1.17 & 42.47 $\pm$ 1.15 & 46.70 $\pm$ 1.53 & 43.16 $\pm$ 0.77 & 47.78 $\pm$ 3.77 & 45.72 $\pm$ 0.64 \\
BiC               & 44.70 $\pm$ 2.12 & 59.53 $\pm$ 4.30 & 42.06 $\pm$ 2.41 & 61.45 $\pm$ 6.25 & 42.92 $\pm$ 1.47 & 71.93 $\pm$ 2.45 \\
\cmidrule(lr){1-7} 
\textbf{\memname w/o DA}  & 54.05 $\pm$ 4.94 & 59.47 $\pm$ 0.61 & 60.87 $\pm$ 0.88 & 74.58 $\pm$ 0.60 & 60.92 $\pm$ 6.48 & 83.91 $\pm$ 0.40 \\ 
\textbf{\our}     & \textbf{66.25 $\pm$ 0.21} & 61.91 $\pm$ 0.63 & \textbf{71.13 $\pm$ 0.18} & 76.86 $\pm$ 0.04 & \textbf{73.90 $\pm$ 0.80} & 85.10 $\pm$ 0.16 \\
\bottomrule
\end{tabular}%
}
\vspace{-1em}
\end{table*}

==> tables/cifar10-blurry10-online.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{graphicx}
% \begin{table}[]
% \centering
% \caption{Comparison of the Last Accuracy (A5, \%) on CIFAR10-Blurry10-Online}
% \label{tab:A5-cifar10-blurry10-online}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{@{}ccccc@{}}
% \toprule
% Methods & None & CutMix & AutoAug & RandAug \\ 
% \midrule
% \multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=200}}\\
% EWC & 40.1 $\pm$ 2.1 & 41.9 $\pm$ 1.1 & 48.3 $\pm$ 3.5 & 44.8 $\pm$ 0.7 \\
% Rwalk & 38.7 $\pm$ 1.5 & 41.5 $\pm$ 2.3 & 48.7 $\pm$ 2.8 & 46.6 $\pm$ 3.0 \\
% iCaRL & 37.4 $\pm$ 1.3 & 38.0 $\pm$ 3.8 & 41.8 $\pm$ 2.4 & 38.4 $\pm$ 1.5\\
% GDumb & 33.4 $\pm$ 2.1 & 35.9 $\pm$ 1.0 & 38.5 $\pm$ 1.1 & 37.2 $\pm$ 2.0 \\
% BiC & 33.3 $\pm$ 0.9 & 33.3 $\pm$ 0.9 & 29.8 $\pm$ 3.2 & 27.2 $\pm$ 2.7 \\
% \textbf{\memname (Ours)} & 45.8 $\pm$ 3.7 & 46.8 $\pm$ 3.2 & 54.1 $\pm$ 1.9 & 51.0 $\pm$ 1.5 \\
% \textbf{\memname (RandAug)} & 44.4 $\pm$ 1.4 & 45.9 $\pm$ 2.4 & 55.4 $\pm$ 2.2 & 49.9 $\pm$ 3.0 \\ 
% \midrule
% \multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=500}}\\
% EWC & 55.7 $\pm$ 4.6 & 56.2 $\pm$ 0.7 & 64.8 $\pm$ 0.6 & 60.1 $\pm$ 5.3 \\
% Rwalk & 53.7 $\pm$ 3.2 & 57.6 $\pm$ 1.4 & 64.8 $\pm$ 1.0 & 62.5 $\pm$ 3.0 \\
% iCaRL & 46.0 $\pm$ 3.0 & 47.0 $\pm$ 1.4 & 51.6 $\pm$ 2.8 & 51.3 $\pm$ 1.2 \\
% GDumb & 46.7 $\pm$ 1.5 & 49.5 $\pm$ 1.1 & 55.9 $\pm$ 1.4 & 54.3 $\pm$ 1.4 \\
% BiC & 42.1 $\pm$ 2.4 & 42.1 $\pm$ 2.4 & 38.7 $\pm$ 1.5 & 38.6 $\pm$ 2.8 \\
% \textbf{\memname (Ours)} & 57.8 $\pm$ 4.5 & 60.7 $\pm$ 3.2 & 70.5 $\pm$ 0.6 & 69.8 $\pm$ 1.3 \\
% \textbf{\memname (RandAug)} & 60.9 $\pm$ 0.9 & 62.1 $\pm$ 3.6 & 69.6 $\pm$ 3.0 & 68.6 $\pm$ 0.7 \\
% \midrule
% \multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=1,000}}\\
% EWC & 68.7 $\pm$ 1.0 & 70.5 $\pm$ 0.7 & 75.1 $\pm$ 2.2 & 73.0 $\pm$ 0.5 \\
% Rwalk & 68.2 $\pm$ 1.9 & 69.7 $\pm$ 1.0 & 76.1 $\pm$ 4.1 & 73.6 $\pm$ 0.1 \\
% iCaRL & 53.6 $\pm$ 2.8 & 56.1 $\pm$ 2.7 & 62.6 $\pm$ 6.2 & 57.7 $\pm$ 0.7 \\
% GDumb & 00.00 & 00.00 & 00.00 & 00.00 \\
% BiC & 47.8 $\pm$ 3.0 & 47.8 $\pm$ 3.0 & 45.7 $\pm$ 5.9 & 45.4 $\pm$ 7.8 \\
% \textbf{\memname (Ours)} & 71.0 $\pm$ 0.9 & 74.0 $\pm$ 0.8 & 78.3 $\pm$ 0.9 & 76.7 $\pm$ 0.9 \\
% \textbf{\memname (RandAug)} & 70.9 $\pm$ 1.6 & 74.8 $\pm$ 0.7 & 77.6 $\pm$ 0.7 & 76.4 $\pm$ 0.4 \\ \bottomrule
% \end{tabular}%
% }
% \end{table}

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{graphicx}
% \begin{table}[]
% \centering
% \caption{Comparison of the Last Forgetting (F5, \%) on CIFAR10-Blurry10-Online}
% \label{tab:F5-cifar10-blurry10-online}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{@{}ccccc@{}}
% \toprule 
% Methods & None & CutMix & AutoAug & RandAug \\ \midrule
% \multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=200}}\\
% EWC                         & 21.2 $\pm$ 0.8 & 24.0 $\pm$ 2.6 & 18.3 $\pm$ 3.1 & 17.9 $\pm$ 2.0 \\
% Rwalk                       & 20.7 $\pm$ 2.4 & 24.0 $\pm$ 3.1 & 18.6 $\pm$ 0.7 & 17.8 $\pm$ 1.6 \\
% iCaRL                       & 2.1  $\pm$ 2.2 & 1.5  $\pm$ 0.4 & 6.0  $\pm$ 1.8 & 4.8  $\pm$ 3.2 \\
% GDumb                       & 1.7  $\pm$ 3.0 & 1.7  $\pm$ 3.5 & 3.5  $\pm$ 2.5 & 3.4  $\pm$ 3.9 \\
% BiC                         & 3.9  $\pm$ 1.6 & 3.9  $\pm$ 1.6 & 10.5 $\pm$ 3.9 & 8.1  $\pm$ 1.8 \\
% \textbf{\memname (Ours)}    & 0.8  $\pm$ 3.3 & 1.1  $\pm$ 0.8 & -1.3 $\pm$ 1.9 & 1.3  $\pm$ 0.6 \\
% \textbf{\memname (RandAug)} & 0.9  $\pm$ 0.9 & 0.5  $\pm$ 0.9 & -1.9 $\pm$ 1.1  & -0.7$\pm$ 2.0 \\ \midrule
% \multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=500}}\\
% EWC   & 16.1 $\pm$ 3.9 & 20.2 $\pm$ 0.5 & 12.3 $\pm$ 4.0  & 13.8 $\pm$ 3.9 \\
% Rwalk & 17.0 $\pm$ 0.3 & 21.0 $\pm$ 0.9 & 11.9 $\pm$ 3.1 & 12.0 $\pm$ 0.9 \\
% iCaRL & 4.8 $\pm$ 1.7 & 4.8 $\pm$ 2.6 & 6.9 $\pm$ 2.4 & 4.3 $\pm$ 3.6 \\
% GDumb & -1.7 $\pm$ 0.9 & 1.4 $\pm$ 2.8 & -1.6 $\pm$ 0.7 & -1.8 $\pm$ 1.0 \\
% BiC   & 1.3 $\pm$ 2.3 & 1.3 $\pm$ 2.3 & 11.0 $\pm$ 7.8 & 6.23 $\pm$ 1.0 \\
% \textbf{\memname (Ours)} & 0.2 $\pm$ 1.4 & -0.2 $\pm$ 1.1 & -1.2 $\pm$ 0.5 & -1.4 $\pm$ 1.2 \\
% \textbf{\memname (RandAug)} & 1.0 $\pm$ 1.1 & 0.0 $\pm$ 1.1 & -0.5 $\pm$ 0.9 & -1.6 $\pm$ 2.0 \\ \midrule
% \multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=1000}}\\
% EWC   & 12.6 $\pm$ 1.8 & 14.5 $\pm$ 1.6 & 10.1 $\pm$ 1.0 & 11.3 $\pm$ 0.7 \\
% Rwalk & 11.5 $\pm$ 1.2  & 15.7 $\pm$ 2.5 & 10.2 $\pm$ 1.5 & 10.5 $\pm$ 0.7 \\
% iCaRL & 7.2 $\pm$ 2.6 & 6.2 $\pm$ 2.7 & 8.9 $\pm$ 0.2 & 6.9 $\pm$ 2.3 \\
% GDumb & 00.00 & 00.00 & 00.00 & 00.00 \\
% BiC   & 3.0 $\pm$ 1.4 & 3.0 $\pm$ 1.4 & 10.7 $\pm$ 1.8 & 9.1 $\pm$ 4.4 \\
% \textbf{\memname (Ours)} & -1.5 $\pm$ 1.3 & -0.2 $\pm$ 0.9 & 0.9 $\pm$ 0.8 & -0.5 $\pm$ 1.6 \\
% \textbf{\memname (RandAug)} & -1.4 $\pm$ 0.7 & -0.2 $\pm$ 0.8 & 0.3 $\pm$ 0.9 & 0.8 $\pm$ 1.1 \\ \bottomrule
% \end{tabular}%
% }
% \end{table}

% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{graphicx}
% \begin{table}[]
% \centering
% \caption{Comparison of the Intransigence (I5, \%) on CIFAR10-Blurry10-Online}
% \label{tab:I5-cifar10-blurry10-online}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{@{}ccccc@{}}
% \toprule
% Methods & None & CutMix & AutoAug & RandAug \\ \midrule
% \multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=200}}\\
% EWC & 61.9 $\pm$ 4.5 & 48.4 $\pm$ 28.1 & 51.3 $\pm$ 10.1 & 57.7 $\pm$ 8.8 \\
% Rwalk & 65.8 $\pm$ 4.9 & 48.7 $\pm$ 27.1 & 48.9 $\pm$ 6.3 & 58.9 $\pm$ 8.1 \\
% iCaRL & 63.5 $\pm$ 13.7 & 50.3 $\pm$ 5.3 & 44.9 $\pm$ 11.5 & 67.7 $\pm$ 3.0 \\
% GDumb & 64.3 $\pm$ 11.6 & 55.3 $\pm$ 6.0 & 54.1 $\pm$ 16.1& 58.7 $\pm$ 12.8  \\
% BiC & 50.4 $\pm$ 7.0 & 50.4 $\pm$ 7.0 & 52.5 $\pm$ 23.2 & 73.8 $\pm$ 18.5 \\
% \textbf{\memname (Ours)} & 52.7 $\pm$ 10.7 & 52.4 $\pm$ 9.1 & 37.5 $\pm$ 10.9 & 40.5 $\pm$ 8.2 \\
% \textbf{\memname (RandAug)} & 49.5 $\pm$ 11.1 & 49.4 $\pm$ 11.9 & 38.2 $\pm$ 8.2 & 45.3 $\pm$ 13.7 \\ \midrule
% \multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=500}}\\
% EWC & 44.2 $\pm$ 12.0 & 34.3 $\pm$ 11.4 & 29.1 $\pm$ 9.8 & 34.4 $\pm$ 11.4 \\
% Rwalk & 45.8 $\pm$ 9.8 & 38.1 $\pm$ 13.8 & 28.3 $\pm$ 8.6 & 29.7 $\pm$ 8.5 \\
% iCaRL & 51.9 $\pm$ 2.6 & 44.6 $\pm$ 16.8 & 40.3 $\pm$ 9.2 & 46.8 $\pm$ 3.9 \\
% GDumb & 48.1 $\pm$ 16.3 & 40.9 $\pm$ 14.0 & 40.0 $\pm$ 14.6 & 37.8 $\pm$ 11.8 \\
% BiC & 52.0 $\pm$ 15.5 & 52.0 $\pm$ 15.5 & 58.4 $\pm$ 24.8 & 58.7 $\pm$ 8.9 \\
% \textbf{\memname (Ours)} & 39.6 $\pm$ 14.3 & 40.4 $\pm$ 18.3  & 25.3 $\pm$ 9.9 & 22.5 $\pm$ 9.1 \\
% \textbf{\memname (RandAug)} & 35.7 $\pm$ 13.9 & 38.4 $\pm$ 15.8 & 22.6 $\pm$ 9.2 & 24.1 $\pm$ 7.4 \\ \midrule
%  \multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=1000}}\\
% EWC & 26.0 $\pm$ 10.9 & 19.6 $\pm$ 12.1 & 22.3 $\pm$ 10.1 & 25.0 $\pm$ 8.8 \\
% Rwalk & 25.2 $\pm$ 11.6 & 23.6 $\pm$ 16.4 & 19.9 $\pm$ 9.3 & 19.4 $\pm$ 6.1 \\
% iCaRL & 37.8 $\pm$ 13.5 & 45.1 $\pm$ 15.6 & 38.1 $\pm$ 18.3 & 41.7 $\pm$ 9.6 \\
% GDumb & 00.00 & 00.00 & 00.00 & 00.00 \\
% BiC & 52.8 $\pm$ 15.5 & 52.8 $\pm$ 15.5 & 51.4 $\pm$ 37.5 & 40.0 $\pm$ 21.9  \\
% \textbf{\memname (Ours)} & 21.7 $\pm$ 12.3 & 21.2 $\pm$ 12.2 & 13.1 $\pm$ 6.2 & 15.6 $\pm$ 6.9 \\
% \textbf{\memname (RandAug)} & 22.1 $\pm$ 14.1 & 20.0 $\pm$ 9.0 & 10.5 $\pm$ 6.7 & 13.9 $\pm$ 7.2 \\ \bottomrule
% \end{tabular}%
% }
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}



% \begin{table}[t]
% \centering
% \caption{Comparison with three metrics (A5, F5, and I5: \%) for three episodic memory sizes in CIFAR10-Blurry10-Online. DA is used in \our denotes CutMix+AutoAug.}
% \label{tab:cifar10-blurry10-online}
% % \resizebox{\linewidth}{!}{%
% \begin{tabular}{@{}crrr@{}}
% \toprule
% % Methods & \multicolumn{3}{c}{$K$=200} \\ \midrule
% %  & A5 (\uparrow) & F5 (\downarrow) & I5 (\downarrow) \\
% Methods & A5 ($\uparrow$) & F5 ($\downarrow$) & I5 ($\downarrow$) \\ \midrule
% \multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=200}}\\
% EWC & 40.07 $\pm$ 2.14 & 21.20 $\pm$ 0.76  & 61.91 $\pm$ 4.51 \\
% Rwalk & 38.66 $\pm$ 1.52 & 20.67 $\pm$ 2.36 & 65.81 $\pm$ 4.85 \\
% iCaRL & 37.43 $\pm$ 1.31 & 2.08 $\pm$ 2.23 & 63.51 $\pm$ 13.73 \\
% GDumb & 35.85 $\pm$ 1.03 & 1.67 $\pm$ 3.49 &  55.31 $\pm$ 6.02 \\
% BiC & 33.29 $\pm$ 0.86 & 3.91 $\pm$ 1.64 & 50.37 $\pm$ 6.96\\ 
% \cmidrule(lr){1-4} 
% \textbf{\memname} & 44.41 $\pm$ 1.40 & 0.90 $\pm$ 0.93 & 49.51 $\pm$ 11.09 \\
% \textbf{\our} & \textbf{54.61 $\pm$ 1.62} & \textbf{-2.60 $\pm$ 1.91} & \textbf{43.57 $\pm$ 11.63} \\ \midrule
% % Methods & \multicolumn{3}{c}{$K$=500} \\ \midrule
% %  & A5 & F5 & I5 \\
% % Methods & A5 ($\uparrow$) & F5 ($\downarrow$) & I5 ($\downarrow$) \\ \midrule
% \multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=500}}\\
% EWC & 55.65 $\pm$ 4.60 & 16.06 $\pm$ 3.89 & 44.24 $\pm$ 11.98 \\
% Rwalk & 53.66 $\pm$ 3.18 & 17.04 $\pm$ 0.31 & 45.81 $\pm$ 9.78 \\
% iCaRL & 45.98 $\pm$ 3.04 & 4.75 $\pm$ 1.70 & 51.91 $\pm$ 2.57 \\
% GDumb & 49.47 $\pm$ 1.08 & 1.44 $\pm$ 2.77 & 40.91 $\pm$ 14.04 \\
% BiC & 42.06 $\pm$ 2.41 & 1.34 $\pm$ 2.27 & 52.04 $\pm$ 15.50 \\
% \cmidrule(lr){1-4} 
% \textbf{\memname} & 60.87 $\pm$ 0.88 & 0.95 $\pm$ 1.14 & 35.74 $\pm$ 13.89 \\
% \textbf{\our} & \textbf{71.13 $\pm$ 0.25} & \textbf{-0.85 $\pm$ 0.28} & \textbf{18.29 $\pm$ 14.21} \\ \midrule
% % Methods & \multicolumn{3}{c}{$K$=1000} \\ \midrule
% %  & A5 & F5 & I5 \\
% % Methods & A5 ($\uparrow$) & F5 ($\downarrow$) & I5 ($\downarrow$) \\ \midrule
% \multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=1000}}\\
% EWC & 68.67 $\pm$ 0.95 & 12.63 $\pm$ 1.78 & 25.97 $\pm$ 10.88 \\
% Rwalk & 68.20 $\pm$ 1.86 & 11.48 $\pm$ 1.19 & 25.17 $\pm$ 11.57 \\
% iCaRL & 53.60 $\pm$ 2.82 & 7.21 $\pm$ 2.58 & 37.84 $\pm$ 13.49 \\
% GDumb & 64.26 $\pm$ 1.21 & 0.37 $\pm$ 1.92 & 31.81 $\pm$ 13.37 \\
% BiC & 47.81 $\pm$ 3.04 & 3.03 $\pm$ 1.44 & 52.77 $\pm$ 15.54 \\
% \cmidrule(lr){1-4} 
% \textbf{\memname} & 70.93 $\pm$ 1.57 & \textbf{-1.43 $\pm$ 0.71} & 22.07 $\pm$ 14.07 \\
% \textbf{\our} & \textbf{78.04 $\pm$ 0.50} & 1.29 $\pm$ 1.26 & \textbf{11.64 $\pm$ 5.83} \\ \bottomrule
% \end{tabular}
% % }
% \vspace{-3mm}
% \end{table}


\begin{table*}[t]
\centering
\caption{Comparison with three metrics (A5, F5, and I5: \%) for three episodic memory sizes in CIFAR10-Blurry10-Online. DA is used in \our denotes CutMix+AutoAug.}
\label{tab:cifar10-blurry10-online}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}crrrrrrrrr@{}}
\toprule
& \multicolumn{3}{c}{ { K=200}} & \multicolumn{3}{c}{ { K=500}} & \multicolumn{3}{c}{ { K=1,000}} \\
% Methods & \multicolumn{3}{c}{$K$=200} \\ \midrule
%  & A5 (\uparrow) & F5 (\downarrow) & I5 (\downarrow) \\
Methods & A5 ($\uparrow$) & F5 ($\downarrow$) & I5 ($\downarrow$) & A5 ($\uparrow$) & F5 ($\downarrow$) & I5 ($\downarrow$) & A5 ($\uparrow$) & F5 ($\downarrow$) & I5 ($\downarrow$) \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
% \multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=200}}\\
EWC & 40.07 $\pm$ 2.14 & 21.20 $\pm$ 0.76  & 61.91 $\pm$ 4.51 & 55.65 $\pm$ 4.60 & 16.06 $\pm$ 3.89 & 44.24 $\pm$ 11.98 & 68.67 $\pm$ 0.95 & 12.63 $\pm$ 1.78 & 25.97 $\pm$ 10.88 \\
Rwalk & 38.66 $\pm$ 1.52 & 20.67 $\pm$ 2.36 & 65.81 $\pm$ 4.85 & 53.66 $\pm$ 3.18 & 17.04 $\pm$ 0.31 & 45.81 $\pm$ 9.78 & 68.20 $\pm$ 1.86 & 11.48 $\pm$ 1.19 & 25.17 $\pm$ 11.57 \\
iCaRL & 37.43 $\pm$ 1.31 & 2.08 $\pm$ 2.23 & 63.51 $\pm$ 13.73 &  45.98 $\pm$ 3.04 & 4.75 $\pm$ 1.70 & 51.91 $\pm$ 2.57 & 53.60 $\pm$ 2.82 & 7.21 $\pm$ 2.58 & 37.84 $\pm$ 13.49 \\
GDumb & 35.85 $\pm$ 1.03 & 1.67 $\pm$ 3.49 &  55.31 $\pm$ 6.02 & 49.47 $\pm$ 1.08 & 1.44 $\pm$ 2.77 & 40.91 $\pm$ 14.04 & 64.26 $\pm$ 1.21 & 0.37 $\pm$ 1.92 & 31.81 $\pm$ 13.37\\
BiC & 33.29 $\pm$ 0.86 & 3.91 $\pm$ 1.64 & 50.37 $\pm$ 6.96  & 42.06 $\pm$ 2.41 & 1.34 $\pm$ 2.27 & 52.04 $\pm$ 15.50 & 47.81 $\pm$ 3.04 & 3.03 $\pm$ 1.44 & 52.77 $\pm$ 15.54 \\ 
\cmidrule(lr){1-10} 
\textbf{\memname w/o DA} & 44.41 $\pm$ 1.40 & 0.90 $\pm$ 0.93 & 49.51 $\pm$ 11.09  & 60.87 $\pm$ 0.88 & 0.95 $\pm$ 1.14 & 35.74 $\pm$ 13.89 & 70.93 $\pm$ 1.57 & \textbf{-1.43 $\pm$ 0.71} & 22.07 $\pm$ 14.07 \\
\textbf{\memname} & \textbf{54.61 $\pm$ 1.62} & \textbf{-2.60 $\pm$ 1.91} & \textbf{43.57 $\pm$ 11.63} & \textbf{71.13 $\pm$ 0.25} & \textbf{-0.85 $\pm$ 0.28} & \textbf{18.29 $\pm$ 14.21} & \textbf{78.04 $\pm$ 0.50} & 1.29 $\pm$ 1.26 & \textbf{11.64 $\pm$ 5.83}\\ \bottomrule
\end{tabular}
}
\end{table*}

==> tables/imagenet-blurry10-online.tex <==
\begin{table}[]
\centering
\caption{Comparison with three metrics (A5, F5, and I5: \%) in ImageNet-Blurry10-Online.}
\label{tab:imagenet-blurry10-online}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}crrr@{}}
\toprule
Methods & A5 ($\uparrow$) & F5 ($\downarrow$) & I5 ($\downarrow$) \\ \midrule
\multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=500}}\\
%  \multicolumn{3}{c}{K=2000}\\
EWC & 39.54 & 14.41 & 42.68 \\
Rwalk & 35.26 & 13.92 & 46.96 \\
iCaRL & 17.52 & 1.94 & 81.94 \\
GDumb & 21.52 & 4.07 & 60.70 \\
BiC & 1.78 & 9.45 & 80.44 \\
BiC^* & 0.00 & 0.00 & 0.00 \\
\cmidrule(lr){1-4} 
\textbf{\memname} & 37.96 & 2.63 & 44.26 \\
\textbf{\our} & \textbf{50.11} & \textbf{1.39} & \textbf{32.11} \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/mnist-blurry10-online.tex <==
\begin{table}[]
\centering
\caption{Comparison with three metrics (A5, F5, and I5: \%) in MNIST-Blurry10-Online.}
\label{tab:mnist-blurry10-online}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}crrr@{}}
\toprule
Methods & A5 ($\uparrow$) & F5 ($\downarrow$) & I5 ($\downarrow$) \\ \midrule
\multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=500}}\\
%  \multicolumn{3}{c}{K=2000}\\
EWC & 90.98 $\pm$ 0.61 & 4.23 $\pm$ 0.45 & 4.54 $\pm$ 0.94 \\
Rwalk & 90.69 $\pm$ 0.62 & 4.77 $\pm$ 0.36 & 4.96 $\pm$ 0.56 \\
iCaRL & 78.09 $\pm$ 0.60 & 6.09 $\pm$ 0.23 & 17.03 $\pm$ 0.60 \\
GDumb & 88.51 $\pm$ 0.52 & 2.67 $\pm$ 0.31 & 6.75 $\pm$ 0.43 \\
BiC & 77.75 $\pm$ 1.27 & 8.25 $\pm$ 1.45 & 17.37 $\pm$ 1.27 \\
\cmidrule(lr){1-4} 
\textbf{\memname} & \textbf{92.65 $\pm$ 0.33} & \textbf{0.58 $\pm$ 0.09} & \textbf{3.14 $\pm$ 0.94} \\
\textbf{\our} & 91.80 $\pm$ 0.69 & 0.75 $\pm$ 0.30 & 3.62 $\pm$ 0.63 \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/old_cifar10-blurry10-online.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{The Last Accuracy (\%) for CIFAR10-Blurry10-Online over Various Memory-Sizes and  Augmentations. \yj{표를 분리해야 할 거 같네요 글씨가 너무 작음.}}
\label{tab:cifar10-blurry10-online}
\resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lrrlr|rrrr|rrrr@{}}
\begin{tabular}{@{}cccccccccccccc@{}}
\toprule
\multicolumn{2}{c} {Blurry10-Online} & \multicolumn{4}{c}{K=200} & \multicolumn{4}{c}{K=500} & \multicolumn{4}{c}{K=1000} \\
\multicolumn{2}{c} {Methods} & \multicolumn{1}{c}{None} & \multicolumn{1}{c}{CutMix} & RandAug & \multicolumn{1}{c}{AutoAug} & \multicolumn{1}{c}{None} & \multicolumn{1}{c}{CutMix} & \multicolumn{1}{c}{RandAug} & \multicolumn{1}{c}{AutoAug} & \multicolumn{1}{c}{None} & \multicolumn{1}{c}{CutMix} & \multicolumn{1}{c}{RandAug} & \multicolumn{1}{c}{AutoAug} \\ 
\cmidrule(lr){1-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
\multirow{7}{*}{$A_5$} & EWC & 40.07 $\pm$ 2.14 & 41.92 $\pm$ 1.07 & 44.79 $\pm$ 0.69  & 48.32 $\pm$ 3.51 & 55.65 $\pm$ 4.6 & 56.23 $\pm$ 0.74 & 60.08 $\pm$ 5.34 & 64.84 $\pm$ 0.61 & 68.67 $\pm$ 0.95 & 70.50 $\pm$ 0.68 & 73.02 $\pm$ 0.51 & 75.11 $\pm$ 2.24 \\
& Rwalk & 38.66 $\pm$ 1.52 & 41.35 $\pm$ 2.25 & 46.57 $\pm$ 2.95 & 48.71 $\pm$ 2.76 & 53.66 $\pm$ 3.18 & 57.58 $\pm$ 1.40 & 62.5 $\pm$ 3.02 & 64.76 $\pm$ 1.01 & 68.20 $\pm$ 1.86 & 69.72 $\pm$ 1.02 & 73.56 $\pm$ 0.13 & 76.09 $\pm$ 4.08 \\
& iCaRL & 37.43 $\pm$ 1.31 & 37.99 $\pm$ 3.8 & 38.42 $\pm$ 1.48 & 41.83 $\pm$ 2.36 & 45.98 $\pm$ 3.04 & 46.96 $\pm$ 1.40 & 51.30 $\pm$ 1.15 & 51.62 $\pm$ 2.83 & 53.60 $\pm$ 2.82 & 56.11 $\pm$ 2.69 & 57.70 $\pm$ 0.73 & 62.55 $\pm$ 6.19 \\
% ER-FAIR & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &  & \multicolumn{1}{c}{} & 46.49 & 48.83 & 49.27 & 64.75 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\
& GDumb & 34.12 $\pm$ 2.46 & 35.76 $\pm$ 1.39 & 38.16 $\pm$ 1.87 & 40.13 $\pm$ 2.38 & 44.11 $\pm$ 1.10 & 47.59 $\pm$ 0.65 & 53.22 $\pm$ 3.23 & 55.95 $\pm$ 1.08 & 57.91 $\pm$ 1.64 & 62.59 $\pm$ 0.99 & 68.25 $\pm$ 1.68 & 67.26 $\pm$ 1.66 \\
& BiC & \multicolumn{1}{c}{33.29 $\pm$ 0.86} & \multicolumn{1}{c}{33.29 $\pm$ 0.86} & 27.16 $\pm$ 2.71 & \multicolumn{1}{c}{29.79 $\pm$ 3.17} & \multicolumn{1}{c}{42.06 $\pm$ 2.41} & \multicolumn{1}{c}{42.06 $\pm$ 2.41} & \multicolumn{1}{c}{38.62 $\pm$ 2.82} & \multicolumn{1}{c}{38.70 $\pm$ 1.50} & \multicolumn{1}{c}{47.81 $\pm$ 3.04} & \multicolumn{1}{c}{47.81 $\pm$ 3.04} & \multicolumn{1}{c}{45.38 $\pm$ 7.75} & \multicolumn{1}{c}{45.68 $\pm$ 5.87} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
& \textbf{\memname} (Ours) & \textbf{45.82 $\pm$ 3.68} & \textbf{46.82 $\pm$ 3.19} & \multicolumn{1}{r}{\textbf{50.97 $\pm$ 1.53}} & \textbf{54.07 $\pm$ 1.86} & \textbf{57.81 $\pm$ 4.45} & \textbf{60.69 $\pm$ 3.23} & \textbf{69.80 $\pm$ 1.26} & \textbf{70.47 $\pm$ 0.62} & \textbf{70.95 $\pm$ 0.90} & \textbf{74.01 $\pm$ 0.83} & \textbf{76.69 $\pm$ 0.93} & \textbf{78.27 $\pm$ 0.93}\\
& \textbf{\memname} (RandAug) & \textbf{44.41 $\pm$ 1.40} & \textbf{45.90 $\pm$ 2.42} & \multicolumn{1}{r}{\textbf{49.92 $\pm$ 2.97}} & \textbf{55.37 $\pm$ 2.23} & \textbf{60.87 $\pm$ 0.88} & \textbf{62.05 $\pm$ 3.59} & \textbf{68.61 $\pm$ 0.73} & \textbf{69.64 $\pm$ 2.95} & \textbf{70.93 $\pm$ 1.57} & \textbf{74.76 $\pm$ 0.69} & \textbf{76.40 $\pm$ 0.38} & \textbf{77.55 $\pm$ 0.71}\\

\midrule

\multirow{7}{*}{$F_5$} & EWC & 40.07 $\pm$ 2.14 & 41.92 $\pm$ 1.07 & 44.79 $\pm$ 0.69  & 48.32 $\pm$ 3.51 & 55.65 $\pm$ 4.6 & 56.23 $\pm$ 0.74 & 60.08 $\pm$ 5.34 & 64.84 $\pm$ 0.61 & 68.67 $\pm$ 0.95 & 70.50 $\pm$ 0.68 & 73.02 $\pm$ 0.51 & 75.11 $\pm$ 2.24 \\
& Rwalk & 38.66 $\pm$ 1.52 & 41.35 $\pm$ 2.25 & 46.57 $\pm$ 2.95 & 48.71 $\pm$ 2.76 & 53.66 $\pm$ 3.18 & 57.58 $\pm$ 1.40 & 62.5 $\pm$ 3.02 & 64.76 $\pm$ 1.01 & 68.20 $\pm$ 1.86 & 69.72 $\pm$ 1.02 & 73.56 $\pm$ 0.13 & 76.09 $\pm$ 4.08 \\
& iCaRL & 37.43 $\pm$ 1.31 & 37.99 $\pm$ 3.8 & 38.42 $\pm$ 1.48 & 41.83 $\pm$ 2.36 & 45.98 $\pm$ 3.04 & 46.96 $\pm$ 1.40 & 51.30 $\pm$ 1.15 & 51.62 $\pm$ 2.83 & 53.60 $\pm$ 2.82 & 56.11 $\pm$ 2.69 & 57.70 $\pm$ 0.73 & 62.55 $\pm$ 6.19 \\
% ER-FAIR & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &  & \multicolumn{1}{c}{} & 46.49 & 48.83 & 49.27 & 64.75 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\
& GDumb & 34.12 $\pm$ 2.46 & 35.76 $\pm$ 1.39 & 38.16 $\pm$ 1.87 & 40.13 $\pm$ 2.38 & 44.11 $\pm$ 1.10 & 47.59 $\pm$ 0.65 & 53.22 $\pm$ 3.23 & 55.95 $\pm$ 1.08 & 57.91 $\pm$ 1.64 & 62.59 $\pm$ 0.99 & 68.25 $\pm$ 1.68 & 67.26 $\pm$ 1.66 \\
& BiC & \multicolumn{1}{c}{33.29 $\pm$ 0.86} & \multicolumn{1}{c}{33.29 $\pm$ 0.86} & 27.16 $\pm$ 2.71 & \multicolumn{1}{c}{29.79 $\pm$ 3.17} & \multicolumn{1}{c}{42.06 $\pm$ 2.41} & \multicolumn{1}{c}{42.06 $\pm$ 2.41} & \multicolumn{1}{c}{38.62 $\pm$ 2.82} & \multicolumn{1}{c}{38.70 $\pm$ 1.50} & \multicolumn{1}{c}{47.81 $\pm$ 3.04} & \multicolumn{1}{c}{47.81 $\pm$ 3.04} & \multicolumn{1}{c}{45.38 $\pm$ 7.75} & \multicolumn{1}{c}{45.68 $\pm$ 5.87} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
& \textbf{\memname} (Ours) & \textbf{45.82 $\pm$ 3.68} & \textbf{46.82 $\pm$ 3.19} & \multicolumn{1}{r}{\textbf{50.97 $\pm$ 1.53}} & \textbf{54.07 $\pm$ 1.86} & \textbf{57.81 $\pm$ 4.45} & \textbf{60.69 $\pm$ 3.23} & \textbf{69.80 $\pm$ 1.26} & \textbf{70.47 $\pm$ 0.62} & \textbf{70.95 $\pm$ 0.90} & \textbf{74.01 $\pm$ 0.83} & \textbf{76.69 $\pm$ 0.93} & \textbf{78.27 $\pm$ 0.93}\\
& \textbf{\memname} (RandAug) & \textbf{44.41 $\pm$ 1.40} & \textbf{45.90 $\pm$ 2.42} & \multicolumn{1}{r}{\textbf{49.92 $\pm$ 2.97}} & \textbf{55.37 $\pm$ 2.23} & \textbf{60.87 $\pm$ 0.88} & \textbf{62.05 $\pm$ 3.59} & \textbf{68.61 $\pm$ 0.73} & \textbf{69.64 $\pm$ 2.95} & \textbf{70.93 $\pm$ 1.57} & \textbf{74.76 $\pm$ 0.69} & \textbf{76.40 $\pm$ 0.38} & \textbf{77.55 $\pm$ 0.71}\\

\midrule

\multirow{7}{*}{$I_5$} & EWC & 40.07 $\pm$ 2.14 & 41.92 $\pm$ 1.07 & 44.79 $\pm$ 0.69  & 48.32 $\pm$ 3.51 & 55.65 $\pm$ 4.6 & 56.23 $\pm$ 0.74 & 60.08 $\pm$ 5.34 & 64.84 $\pm$ 0.61 & 68.67 $\pm$ 0.95 & 70.50 $\pm$ 0.68 & 73.02 $\pm$ 0.51 & 75.11 $\pm$ 2.24 \\
& Rwalk & 38.66 $\pm$ 1.52 & 41.35 $\pm$ 2.25 & 46.57 $\pm$ 2.95 & 48.71 $\pm$ 2.76 & 53.66 $\pm$ 3.18 & 57.58 $\pm$ 1.40 & 62.5 $\pm$ 3.02 & 64.76 $\pm$ 1.01 & 68.20 $\pm$ 1.86 & 69.72 $\pm$ 1.02 & 73.56 $\pm$ 0.13 & 76.09 $\pm$ 4.08 \\
& iCaRL & 37.43 $\pm$ 1.31 & 37.99 $\pm$ 3.8 & 38.42 $\pm$ 1.48 & 41.83 $\pm$ 2.36 & 45.98 $\pm$ 3.04 & 46.96 $\pm$ 1.40 & 51.30 $\pm$ 1.15 & 51.62 $\pm$ 2.83 & 53.60 $\pm$ 2.82 & 56.11 $\pm$ 2.69 & 57.70 $\pm$ 0.73 & 62.55 $\pm$ 6.19 \\
% ER-FAIR & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &  & \multicolumn{1}{c}{} & 46.49 & 48.83 & 49.27 & 64.75 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\
& GDumb & 34.12 $\pm$ 2.46 & 35.76 $\pm$ 1.39 & 38.16 $\pm$ 1.87 & 40.13 $\pm$ 2.38 & 44.11 $\pm$ 1.10 & 47.59 $\pm$ 0.65 & 53.22 $\pm$ 3.23 & 55.95 $\pm$ 1.08 & 57.91 $\pm$ 1.64 & 62.59 $\pm$ 0.99 & 68.25 $\pm$ 1.68 & 67.26 $\pm$ 1.66 \\
& BiC & \multicolumn{1}{c}{33.29 $\pm$ 0.86} & \multicolumn{1}{c}{33.29 $\pm$ 0.86} & 27.16 $\pm$ 2.71 & \multicolumn{1}{c}{29.79 $\pm$ 3.17} & \multicolumn{1}{c}{42.06 $\pm$ 2.41} & \multicolumn{1}{c}{42.06 $\pm$ 2.41} & \multicolumn{1}{c}{38.62 $\pm$ 2.82} & \multicolumn{1}{c}{38.70 $\pm$ 1.50} & \multicolumn{1}{c}{47.81 $\pm$ 3.04} & \multicolumn{1}{c}{47.81 $\pm$ 3.04} & \multicolumn{1}{c}{45.38 $\pm$ 7.75} & \multicolumn{1}{c}{45.68 $\pm$ 5.87} \\
\cmidrule(lr){2-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
& \textbf{\memname} (Ours) & \textbf{45.82 $\pm$ 3.68} & \textbf{46.82 $\pm$ 3.19} & \multicolumn{1}{r}{\textbf{50.97 $\pm$ 1.53}} & \textbf{54.07 $\pm$ 1.86} & \textbf{57.81 $\pm$ 4.45} & \textbf{60.69 $\pm$ 3.23} & \textbf{69.80 $\pm$ 1.26} & \textbf{70.47 $\pm$ 0.62} & \textbf{70.95 $\pm$ 0.90} & \textbf{74.01 $\pm$ 0.83} & \textbf{76.69 $\pm$ 0.93} & \textbf{78.27 $\pm$ 0.93}\\
& \textbf{\memname} (RandAug) & \textbf{44.41 $\pm$ 1.40} & \textbf{45.90 $\pm$ 2.42} & \multicolumn{1}{r}{\textbf{49.92 $\pm$ 2.97}} & \textbf{55.37 $\pm$ 2.23} & \textbf{60.87 $\pm$ 0.88} & \textbf{62.05 $\pm$ 3.59} & \textbf{68.61 $\pm$ 0.73} & \textbf{69.64 $\pm$ 2.95} & \textbf{70.93 $\pm$ 1.57} & \textbf{74.76 $\pm$ 0.69} & \textbf{76.40 $\pm$ 0.38} & \textbf{77.55 $\pm$ 0.71}\\

\bottomrule
\end{tabular}%
}
\end{table*}

==> tables/uncertainty_measure.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table}[]
% \centering
% \caption{Comparison of Uncertainty Measures.}
% \label{tab:uncertainty}
% \begin{tabular}{llll}
% \hline
%  & Single & VR\_RandAug & VR\_Manual (Ours) \\ \hline
% \textbf{\memname} & 58.59 & 61.27 & 54.2 \\ \hline
% \end{tabular}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[h]
\centering
\caption{Comparison of uncertainty measures for \memname on CIFAR10-Blurry10-Online (K=500).}
\label{tab:unceratinty_measure}
\resizebox{0.8\linewidth}{!}{%
\begin{tabular}{@{}crrr@{}}
\toprule
       & No\_MC & RandAug\_MC & AutoAug\_MC \\ \midrule
% \multicolumn{4}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=500}}\\
A5 (\%) & 58.59  & 61.27       & 60.1  \\ \bottomrule
\end{tabular}%
}
\vspace{-0.5em}
\end{table}

==> tables/various-dataset-blurry10-online.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[]
% \centering
% \caption{Comparison of Last Accuracy (A5, \%) on CIFAR100-Blurry10-Online.}
% \label{tab:cifar100-blurry10-online}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{@{}ccccc@{}}
% \toprule
%  & \multicolumn{4}{c}{K=2000} \\
% Methods & None & CutMix & RandAug & AutoAug \\ 
% \cmidrule(lr){1-1} \cmidrule(lr){2-5}
% EWC & $26.95 \pm 0.36$ & $24.57 \pm 0.17$ & $19.34 \pm 15.89$ & $28.06 \pm 1.41$ \\
% Rwalk & 32.32 $\pm$ 0.78 & 34.41 $\pm$ 0.93 & 35.19 $\pm$ 1.07 & 33.44 $\pm$ 1.73 \\
% iCaRL & 17.39 $\pm$ 1.04 & 19.18 $\pm$ 2.57 & 18.28 $\pm$ 2.45 & 18.91 $\pm$ 0.56 \\
% GDumb & 22.66 $\pm$ 0.76 & 27.45 $\pm$ 0.96 & 28.96 $\pm$ 1.01 & 27.95 $\pm$ 0.76 \\
% BiC & 13.01 $\pm$ 0.24 & 13.01 $\pm$ 0.24 & 14.95 $\pm$ 0.69 &  15.77 $\pm$ 0.70 \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-5}
% \textbf{\memname} & \textbf{34.09 $\pm$ 1.41} & \textbf{37.22 $\pm$ 0.60} & \textbf{37.81 $\pm$ 0.96} & \textbf{38.29 $\pm$ 0.36} \\ \bottomrule
% \end{tabular}%
% }
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{Comparison with three metrics (A\{5, 10\}, F\{5, 10\}, and I\{5, 10\}: \%) in \{MNIST, CIFAR100, ImageNet\}-Blurry10-Online. 
\newline $^*$ indicates the reproduction of BiC with only using classification loss without distilling loss to be better suited for Blurry10 setup.}
\label{tab:various-dataset-blurry10-online}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}crrrrrrlll@{}}
\toprule 
& \multicolumn{3}{c}{MNIST (K=500)} & \multicolumn{3}{c}{CIFAR100 (K=2,000)}  & \multicolumn{3}{c}{ImageNet (K=20,000)} \\ 
Methods & \multicolumn{1}{c}{A5 ($\uparrow$)} & \multicolumn{1}{c}{F5 ($\downarrow$)} & \multicolumn{1}{c}{I5 ($\downarrow$)} & \multicolumn{1}{c}{A5 ($\uparrow$)} & \multicolumn{1}{c}{F5 ($\downarrow$)} & \multicolumn{1}{c}{I5 ($\downarrow$)} & \multicolumn{1}{c}{A10 ($\uparrow$)} & \multicolumn{1}{c}{F10 ($\downarrow$)} & \multicolumn{1}{c}{I10 ($\downarrow$)} \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} 

% & \multicolumn{3}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=500}} & \multicolumn{3}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=2000}} & \multicolumn{3}{l}{\footnotesize \bf {\fontfamily{lmss}\selectfont \hspace{-0.5em} K=20000}}\\
%  \multicolumn{3}{c}{K=2000}\\
EWC & 90.98 $\pm$ 0.61 & 4.23 $\pm$ 0.45 & 4.54 $\pm$ 0.94 & 26.95 $\pm$ 0.36 & 11.47 $\pm$ 1.26 & 43.18 $\pm$ 14.22 & 39.54 & 14.41 & 42.68 \\
Rwalk & 90.69 $\pm$ 0.62 & 4.77 $\pm$ 0.36 & 4.96 $\pm$ 0.56 & 32.31 $\pm$ 0.78 & 15.57 $\pm$ 2.17 & 37.18 $\pm$ 10.02 & 35.26 & 13.92 & 46.96 \\
iCaRL & 78.09 $\pm$ 0.60 & 6.09 $\pm$ 0.23 & 17.03 $\pm$ 0.60 & 17.39 $\pm$ 1.04 & 5.38 $\pm$ 0.88 & 44.18 $\pm$  9.29 & 17.52 & 1.94 & 81.94 \\
GDumb & 88.51 $\pm$ 0.52 & 2.67 $\pm$ 0.31 & 6.75 $\pm$ 0.43  & 27.19 $\pm$ 0.65 & 7.49 $\pm$ 0.95 & 41.18 $\pm$  7.23 & 21.52 & 4.07 & 60.70 \\
BiC & 77.75 $\pm$ 1.27 & 8.25 $\pm$ 1.45 & 17.37 $\pm$ 1.27 & 13.01 $\pm$ 0.24 & 4.63 $\pm$ 0.46 & 53.84 $\pm$ 11.85 & 37.20$^*$ & 1.52$^*$ & 45.02$^*$ \\
\cmidrule(lr){1-10} 
\textbf{\memname w/o DA} & \textbf{92.65 $\pm$ 0.33} & \textbf{0.58 $\pm$ 0.09} & \textbf{3.14 $\pm$ 0.94} & 34.09 $\pm$  1.41 & \textbf{4.01 $\pm$ 0.50} & 34.51 $\pm$ 4.58 & 37.96 & 2.63 & 44.26 \\
\textbf{\our} & 91.80 $\pm$ 0.69 & 0.75 $\pm$ 0.30 & 3.62 $\pm$ 0.63 & \textbf{41.35 $\pm$ 0.95} & 4.99 $\pm$  0.89 & \textbf{20.18 $\pm$ 3.06} & \textbf{50.11} & \textbf{1.39} & \textbf{32.11} \\ \bottomrule
\end{tabular}%
}

\end{table*}

